Convolutional Neural Network Compression through Generalized Kronecker Product Decomposition

Modern Convolutional Neural Network (CNN) architectures, despite their superiority in solving various problems, are generally too large to be deployed on resource constrained edge devices. In this paper, we reduce memory usage and floating-point operations required by convolutional layers in CNNs. We compress these layers by generalizing the Kronecker Product Decomposition to apply to multidimensional tensors, leading to the Generalized Kronecker Product Decomposition (GKPD). Our approach yields a plug-and-play module that can be used as a drop-in replacement for any convolutional layer. Experimental results for image classification on CIFAR-10 and ImageNet datasets using ResNet, MobileNetv2 and SeNet architectures substantiate the effectiveness of our proposed approach. We find that GKPD outperforms state-of-the-art decomposition methods including Tensor-Train and Tensor-Ring as well as other relevant compression methods such as pruning and knowledge distillation.

==> experiments_temp.tex <==
 To validate our method, we provide experimental results for image classification tasks on the CIFAR-10 and ImageNet datasets using popular CNN architectures such as ResNet \citep{he2016deep}, MobileNetv2 \citep{sandler2018mobilenetv2} and SeNet \citep{hu2020senet}. 
    The proposed GKPD provides us with a set of possible decompositions depending on the dimensions of Kronecker factors chosen. Hence, we choose configurations that best match the desired compression rates in all the experiments. 
    Table \ref{tbl:cifar10_top1_decompostion} shows the Top-1 accuracy obtained on the CIFAR-10 dataset using a compressed ResNet32 model referred to as ``KronechkerResNet32'' where the GKPD configurations are set to obtain a 5$\times$ compression rate. 
    More details on our configuration selection strategy is provided in the Appendix.
    
    In the following subsections, we first provide the implementation details. Next, we present comparative experiments using different model compression methods followed by compression experiments applied on different architectures. Finally, we present ablation studies for investigating the effect of 
    
    \subsection{Implementation Details}

    All experiments on CIFAR-10 are run for 200 epochs using Stochastic Gradient Descent (SGD). We use a batch size of 128, weight decay of 0.0001, momentum of 0.1 and an initial learning rate of 0.1 that is subsequently reduced by a factor of 10 at epochs 100 and 150. Similarly, experiments on ImageNet are run for 100 epochs using SGD with a batch size of 256, weight decay of 0.0001, momentum of 0.1 and an initial learning rate of 0.1 that is subsequently reduced by a factor of 10 at epochs 30, 60 and 90. 
    
    \subsection{Comparison with other Compression Methods}
    
    In this section we compare GKPD to other compression methods. We conduct our experiments on a range of model architectures to demonstrate GKPDs applicability to both small models, ResNet26 (0.4M parameters) and ResNet32 (0.5M) as well as larger models such as MobileNetv2 (2.3M), ResNet18 (11M), ResNet50 (25.6M) and SeResNet50 (21M)
    
    In Table \ref{tbl:cifar10_top1_decompostion} we compare our method to other tensor decomposition methods using a ResNet32 model pretrained on CIFAR-10.  Namely, Tensor Train, Tensor Ring and Tucker \citep{wang2018wide}.
    % We compress ResNet32 using GKPD and the aformentiioned methods and reduce the number of parameters to around 90K.  
    Notably, GKPD outperforms all other decomposition methods despite having a slightly larger compression factor.
    We attribute the performance of GKPD to its higher representation power. This is reflected in its ability to better reconstruct weight tensors in a pretrained network in comparison to other decomposition methods. In Fig. \ref{fig:reconstruction_loss} we plot the reconstruction errors of GKPD and Tucker decomposition applied to all layers in a ResNet18 model pretrained on ImageNet. In comparison to Tucker, GKPD provides a lower error for all the layers within the network.
    
    \begin{figure}[t]
        \centering
        \includegraphics[width=0.8\columnwidth]{figures/resnet18_reconstruction_errors.pdf}
        \caption{Reconstruction error between convolution tensors in a pretrained ResNet18 model and compressed representations at a $4\times$ compression rate. GKPD always yields a lower reconstruction error than Tucker decomposition}
        \label{fig:reconstruction_loss}
    \end{figure}
    
    \begin{table}[t]
        \resizebox{\columnwidth}{!}{
        \begin{tabular}{@{}lccc@{}}
            \toprule
            Model & Params (M) & Compression & Accuracy (\%) \\
            \midrule
            Resnet32 & 0.46 & 1$\times$ & 92.55   \\
            \midrule
            TuckerResNet32 & 0.09 & 5$\times$ & 87.7 \\
            TensorTrainResNet32  & 0.096 & 4.8$\times$ & 88.3 \\
            TensorRingResNet32 & 0.09 & 5$\times$ & 90.6 \\
            % KroneckerResnet32 & 0.08 & 5.8$\times$   & 88.46  \\ % not with nkp
            % (krank=10)
            KroneckerResNet32  & 0.09 & 5$\times$  & \textbf{91.52} \\
            \bottomrule
        \end{tabular}
        }
        \caption{Top-1 Accuracy on CIFAR-10 of compressed ResNet32 models using various decomposition approaches. }
        \label{tbl:cifar10_top1_decompostion}
    \end{table}
    
    To evaluate the performance of the GKPD method on larger datasets, we use the larger ResNet50 as the baseline and compress it by factors of approximately 2$\times$ and 4$\times$. In Table \ref{tbl:imagenet_top1} we show that GKPD outperforms other compression methods such as pruning (ThiNet) \cite{Luo_ThiNet_2017} and filter sharing (FSNet) \cite{Yang_FSNet_2020} for similar compression rates. 
    
    In Table \ref{tbl:cifar10_top1_distillation}, ResNet26, another relatively small model, is used as the baseline to compare GKPD with knowledge distillation (KD) methods. With less parameters, GKPD outperforms two state-of-the-art KD methods.
    
    \begin{table}[t]
        \resizebox{\columnwidth}{!}{
        \begin{tabular}{@{}lccc@{}}
            \toprule
            Model  & Params (M) & Compression & Accuracy (\%) \\
            \midrule
            ResNet50 & 25.6 & 1$\times$ & 75.99 \\
            \midrule
            % (k-rank=4)
            KroneckerResNet50  & 8.98 & 2.85$\times$ & \textbf{74.10}\\
            FSNet & 13.9 & 2.0$\times$ & 73.11 \\ 
            ThiNet  & 12.38 & 2.0$\times$ & 71.01 \\
            \midrule
            % (k-rank=2) 
            KroneckerResNet50  & 7.0 & 3.6$\times$ & \textbf{72.92} \\
            FSNet  & 8.49 & 3.0$\times$ & 70.36 \\ 
            \bottomrule
        \end{tabular}
        }
        \caption{Top-1 Accuracy on ILSVRC-12 of compressed Resnet50 models}
        \label{tbl:imagenet_top1}
    \end{table}

    \begin{table}[t]
        \resizebox{\columnwidth}{!}{
        \begin{tabular}{@{}lccc@{}}
            \toprule
            Model  & Params (M) & Compression & Accuracy (\%) \\
            \midrule
            ResNet26 & 0.37 & 1$\times$ & 92.94 \\
            \midrule
            \citet{Mirzadeh_Improved_Knowledge_Distillation_via_Teacher_Assistant_2020} & 0.17 & 2.13$\times$ & 91.23 \\
         \citet{Heo_Knowledge_Distillation_with_Adversarial_Samples_Supporting_Decision_2019} & 0.17 & 2.13$\times$ & 90.34 \\
            KroneckerResNet26 & 0.14 & 2.69$\times$ & \textbf{93.16} \\
            \midrule
          \citet{Mirzadeh_Improved_Knowledge_Distillation_via_Teacher_Assistant_2020} & 0.075 & 4.88$\times$ & 88.0 \\
          \citet{Heo_Knowledge_Distillation_with_Adversarial_Samples_Supporting_Decision_2019} & 0.075 & 4.88$\times$ & 87.32 \\
            KroneckerResNet26 & 0.069 & 5.29$\times$ & \textbf{91.28} \\
            \bottomrule
        \end{tabular}
        }
        \caption{Top-1 Accuracy CIFAR-10 of compressed ResNet26 models}
        \label{tbl:cifar10_top1_distillation}
    \end{table}
    
    
    \subsection{Compressing Different Architectures Using GKPD}
    
    To further investigate the effectiveness of GKPD, we compress various model architectures. Namely, ResNet, MobileNetv2 and SEResNet. Our experimental results in Table \ref{tbl:cifar10_top1_different_models} indicate GKPD can be applied to a variety of model architectures. Note that, the much smaller compressed KroneckerMobileNetv2 with 0.39M parameters can outperform the compressed KroneckerResNet18 with 0.48M parameters. 
    
    % Place holder
    \begin{table}[t]
        \resizebox{\columnwidth}{!}{
    \begin{tabular}{@{}lccc@{}}
        \toprule
        Model &  Params (M) & Compression & Accuracy  \\ \midrule
        ResNet18    & 11.17     & 1$\times$ & 95.06 \\
        KroneckerResNet18  & 3.77 & 3.0 & 95.02 \\
        KroneckerResNet18  & 1.70  & 6.6  & 94.72 \\
        KroneckerResNet18  & 0.48  & 23.1  & 92.62 \\
        \midrule
        MobileNetv2 &  2.30 & 1$\times$ & 94.18  \\ 
        KroneckerMobileNetv2 &  0.73 & 3.14  & 93.80\\ 
        KroneckerMobileNetv2 &  0.29 & 7.79 & 93.01 \\
        KroneckerMobileNetv2 & 0.18 & 12.43 & 91.48 \\
        \midrule
        SeResNet50 & 21.40 & 1$\times$ & 95.15 \\
        KroneckerSeResNet50 & 0.93 & 22.96 & 93.66 \\
        KroneckerSeResNet50 & 0.29 & 73.30 & 91.85 \\
    \bottomrule
    \end{tabular}
        }
        \caption{Top-1 Accuracy on CIFAR-10 of compressed models using various compression factors}
        \label{tbl:cifar10_top1_different_models}
    \end{table}
    
    
    \subsection{Ablation studies}
    \begin{table}[t]
        \resizebox{\columnwidth}{!}{
        \begin{tabular}{@{}lll@{}}
        \toprule
        Model & Params (M) &  Accuracy  \\ \midrule
        Resnet18 & 11.17 & 94.47 \\
        \midrule
        KronenckerResnet18 (krank=1) &  0.37 & 90.51 \\
        KronenckerResnet18 (krank=1) + NKP  & 0.37 & 91.12 \\
        KronenckerResnet18 (krank=2) + NKP & 0.37 & 91.86  \\
        KronenckerResnet18 (krank=2) + NKP + KD & 0.37 &\textbf{92.30} \\
        \bottomrule
    \end{tabular}
        }
        \caption{Top-1 image classification accuracy of compressed ResNet18 on CIFAR-10. Here krank denotes the number of terms used in the summation for each layer, NKP refers to initializing the Kronecker factors to be the solutions to the Nearest Kronecker Product problem and KD indicates the use of Knowledge Distillation during training.}
        \label{tbl:cifar-10-ablation}
    \end{table}

==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );
sub makeexternaldocument {
    if (!($root_filename eq $_[0]))
    {
        system( "latexmk -cd -pdf \"$_[0]\"" );
    }
}
